Bilinear Recovery using Adaptive Vector-AMP

We consider the problem of jointly recovering the vector $\boldsymbol{b}$ and the matrix $\boldsymbol{C}$ from noisy measurements $\boldsymbol{Y} = \boldsymbol{A}(\boldsymbol{b})\boldsymbol{C} + \boldsymbol{W}$, where $\boldsymbol{A}(\cdot)$ is a known affine linear function of $\boldsymbol{b}$ (i.e., $\boldsymbol{A}(\boldsymbol{b})=\boldsymbol{A}_0+\sum_{i=1}^Q b_i \boldsymbol{A}_i$ with known matrices $\boldsymbol{A}_i$). This problem has applications in matrix completion, robust PCA, dictionary learning, self-calibration, blind deconvolution, joint-channel/symbol estimation, compressive sensing with matrix uncertainty, and many other tasks. To solve this bilinear recovery problem, we propose the Bilinear Adaptive Vector Approximate Message Passing (BAd-VAMP) algorithm. We demonstrate numerically that the proposed approach is competitive with other state-of-the-art approaches to bilinear recovery, including lifted VAMP and Bilinear GAMP.

==> macros_gen.tex <==
%%USAGE: \input{macrosLatex.tex}

\usepackage{graphicx}
\usepackage{amsmath,bm,cite}
\usepackage{amsmath,mathtools}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{enumerate}
\usepackage{accents}
\usepackage{verbatim}
\usepackage{geometry} % to change the page dimensions
\usepackage{etoolbox}
\usepackage{hyperref}
\usepackage{subcaption}
\usepackage{listings}
\usepackage{bbm}
% \usepackage{color}

\usepackage{algorithm,algpseudocode}% http://ctan.org/pkg/{algorithms,algorithmx}
% \usepackage{algorithmic}
\algnewcommand{\Inputs}[1]{%
  \State \textbf{inputs:}
  \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Initialize}[1]{%
  \State \textbf{initialize:}
  \Statex \hspace*{\algorithmicindent}\parbox[t]{.8\linewidth}{\raggedright #1}
}

% \geometry{letterpaper} % or letterpaper (US) or a5paper or....
\geometry{margin=1in}

\usepackage[usenames]{color}
\usepackage{stmaryrd}
%\graphicspath{ {figures/ortho_bivamp-July25/} }


%-------------------------------------
%Coding
%\lstinputlisting[language=Python]{prob3.py}
%\begin{lstlisting}[language=Python]...\end{lstlisting}

% \definecolor{codegreen}{rgb}{0,0.6,0}
% \definecolor{codegray}{rgb}{0.5,0.5,0.5}
% \definecolor{codepurple}{rgb}{0.58,0,0.82}
% \definecolor{backcolour}{rgb}{0.95,0.95,0.92}
% \lstdefinestyle{mystyle}{
% backgroundcolor=\color{backcolour},
% commentstyle=\color{codegreen},
% keywordstyle=\color{magenta},
% numberstyle=\tiny\color{codegray},
% stringstyle=\color{codepurple},
% basicstyle=\footnotesize,
% breakatwhitespace=false,
% breaklines=true,
% captionpos=b,
% keepspaces=true,
% numbers=left,
% numbersep=5pt,
% showspaces=false,
% showstringspaces=false,
% showtabs=false,
% tabsize=2
% }

%\usepackage{tikz} 
%\usetikzlibrary{positioning}
%\usetikzlibrary{arrows,calc,decorations.markings,math,arrows.meta}

\newcommand{\Abf}{\bm{A}}
\newcommand{\Ahat}{\widehat{\bm{A}}}
\newcommand{\Bbf}{\bm{B}}
\newcommand{\Xbf}{\bm{X}}
\newcommand{\Xhat}{\widehat{\bm{X}}}
\newcommand{\Qbf}{\bm{Q}}
\newcommand{\Ibf}{\bm{I}}
\newcommand{\Ebf}{\bm{E}}
\newcommand{\Ubf}{\bm{U}}
\newcommand{\Sbf}{\bm{S}}
\newcommand{\Vbf}{\bm{V}}
\newcommand{\Fbf}{\bm{F}}
\newcommand{\Ybf}{\bm{Y}}
\newcommand{\Wbf}{\bm{W}}
\newcommand{\Zbf}{\bm{Z}}
\newcommand{\Dbf}{\bm{D}}
\newcommand{\Zhat}{\widehat{\bm{Z}}}
\newcommand{\Cbf}{\bm{C}}
\newcommand{\Hbf}{\bm{H}}
\newcommand{\Gbf}{\bm{G}}
\newcommand{\Rbf}{\bm{R}}
\newcommand{\Pbf}{\bm{P}}
\newcommand{\Tbf}{\bm{T}}

\newcommand{\ybf}{\bm{y}}
\newcommand{\rbf}{\bm{r}}
\newcommand{\sbf}{\bm{s}}
\newcommand{\xbf}{\bm{x}}
\newcommand{\xhat}{\widehat{\bm{x}}}
\newcommand{\abf}{\bm{a}}
\newcommand{\dbf}{\bm{d}}
\newcommand{\wbf}{\bm{w}}
\newcommand{\hbf}{\bm{h}}
\newcommand{\bbf}{\bm{b}}
\newcommand{\bhat}{\widehat{\bm{b}}}
\newcommand{\cbf}{\bm{c}}
\newcommand{\qbf}{\bm{q}}
\newcommand{\zbf}{\bm{z}}
\newcommand{\ebf}{\bm{e}}
\newcommand{\ubf}{\bm{u}}
\newcommand{\fbf}{\bm{f}}
\newcommand{\vbf}{\bm{v}}
\newcommand{\gbf}{\bm{g}}

% bars, tildas and hats
\newcommand{\Abfbar}{\overline{\bm{A}}}
\newcommand{\Rbftil}{\widetilde{\bm{R}}}
\newcommand{\Rbfbar}{\overline{\bm{R}}}
\newcommand{\rbfbar}{\overline{\bm{r}}}
\newcommand{\rbftil}{\widetilde{\bm{r}}}
\newcommand{\Xbfbar}{\overline{\bm{X}}}
\newcommand{\Wbfbar}{\overline{\bm{W}}}
\newcommand{\Wbftil}{\widetilde{\bm{W}}}
\newcommand{\wbfbar}{\overline{\bm{w}}}
\newcommand{\wbftil}{\widetilde{\bm{w}}}
\newcommand{\xbfbar}{\overline{\bm{x}}}


\newcommand{\gambf}{\bm{\gamma}}
\newcommand{\etabf}{\bm{\eta}}
\newcommand*\dif{\mathop{}\!\mathrm{d}} %differential in integrals
\newcommand{\Sigmat}{\widetilde{\bm{\Sigma}}}
\newcommand{\Sigmabf}{\bm{\Sigma}}
\newcommand{\phibf}{\bm{\phi}}


\def\cov{\mathop{\mathrm{Cov}}}
\newcommand{\textr}[1]{\textcolor{red}{#1}}
\DeclareMathOperator{\diag}{Diag}
\newcommand{\nmse}{{\textsf{NMSE}}}
\newcommand{\defn}{\triangleq}
% \newcommand{\defn}{\coloneqq}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\sup}{sup}
\def\Exp{\mathbb{E}}
\def\var{\mathop{\mathrm{var}}}
\def\vec{\mathop{\mathrm{vec}}}
\def\vect{\mathop{\mathrm{vec}}}
\def\mat{\mathop{\mathrm{mat}}}
\def\mat{\mathop{\mathrm{mat}}}
\def\trace{\mathop{\mathrm{tr}}}
\def\det{\mathop{\mathrm{det}}}
\def\prox{\mathop{\mathrm{prox}}}
\def\limn{\lim_{N \rightarrow \infty}}

% \newcommand{\true}{^{\textsf{true}}}
\newcommand{\true}{^{0}}
\newcommand{\inv}{^{-1}}
\newcommand{\itero}{^{(t-1)}}
\newcommand{\iter}{^{(t)}}
\newcommand{\itern}{^{(t+1)}}
\newcommand{\tran}{^{\textsf{T}}}
\newcommand{\herm}{^{\textsf{H}}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
% \newcommand{\obar}[1]{\overline{#1}}
\newcommand{\MMSE}{{\text{\sf MMSE}}}
\newcommand{\LMMSE}{{\text{\sf LMMSE}}}
\newcommand{\EM}{{\text{\sf EM}}}
\newcommand{\ML}{{\text{\sf ML}}}

\newcommand{\zero}{\bm{0}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\cnormal}{\mathcal{CN}}
\newcommand{\unif}{\mathcal{U}}
\newcommand{\kron}{\otimes}
\newcommand{\ones}{\bm{1}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\thetabf}{\bm{\theta}}
\newcommand{\Thetabf}{\bm{\Theta}}
\newcommand{\betabf}{\bm{\beta}}
\newcommand{\mubf}{\bm{\mu}}

% Probability density notations
\newcommand{\prob}{\mathbb{P}}
\newcommand{\bx}{b_{\textsf{x}}}
\newcommand{\bu}{b_{\textsf{u}}}
\newcommand{\px}{p_{\textsf{x}}}

%% strainght
% \newcommand{\Abf}{\mathbf{A}}
% \newcommand{\Ahat}{\widehat{\mathbf{A}}}
% \newcommand{\Bbf}{\mathbf{B}}
% \newcommand{\Xbf}{\mathbf{X}}
% \newcommand{\Xhat}{\widehat{\mathbf{X}}}
% \newcommand{\Qbf}{\mathbf{Q}}
% \newcommand{\Ibf}{\mathbf{I}}
% \newcommand{\Ebf}{\mathbf{E}}
% \newcommand{\Ubf}{\mathbf{U}}
% \newcommand{\Sbf}{\mathbf{S}}
% \newcommand{\Vbf}{\mathbf{V}}
% \newcommand{\Fbf}{\mathbf{F}}
% \newcommand{\Ybf}{\mathbf{Y}}
% \newcommand{\Wbf}{\mathbf{W}}
% \newcommand{\Wbar}{\overline{\mathbf{W}}}
% \newcommand{\Zbf}{\mathbf{Z}}
% \newcommand{\Dbf}{\mathbf{D}}
% \newcommand{\Zhat}{\widehat{\mathbf{Z}}}
% \newcommand{\Cbf}{\mathbf{C}}
% \newcommand{\Hbf}{\mathbf{H}}
% \newcommand{\Gbf}{\mathbf{G}}
% \newcommand{\Rbf}{\mathbf{R}}
% \newcommand{\Pbf}{\mathbf{P}}
% \newcommand{\Tbf}{\mathbf{T}}
%
% \newcommand{\ybf}{\mathbf{y}}
% \newcommand{\pbf}{\mathbf{p}}
% \newcommand{\rbf}{\mathbf{r}}
% \newcommand{\rtilde}{\widetilde{\mathbf{r}}}
% \newcommand{\sbf}{\mathbf{s}}
% \newcommand{\xbf}{\mathbf{x}}
% \newcommand{\xhat}{\widehat{\mathbf{x}}}
% \newcommand{\abf}{\mathbf{a}}
% \newcommand{\dbf}{\mathbf{d}}
% \newcommand{\wbf}{\mathbf{w}}
% \newcommand{\wtilde}{\widetilde{\mathbf{w}}}
% \newcommand{\hbf}{\mathbf{h}}
% \newcommand{\bbf}{\mathbf{b}}
% \newcommand{\bhat}{\widehat{\mathbf{b}}}
% \newcommand{\cbf}{\mathbf{c}}
% \newcommand{\qbf}{\mathbf{q}}
% \newcommand{\zbf}{\mathbf{z}}
% \newcommand{\ebf}{\mathbf{e}}
% \newcommand{\ubf}{\mathbf{u}}
% \newcommand{\fbf}{\mathbf{f}}
% \newcommand{\vbf}{\mathbf{v}}
% \newcommand{\gbf}{\mathbf{g}}
%
% % bars, tildas and hats
% \newcommand{\Abfbar}{\overline{\mathbf{A}}}
% \newcommand{\Rbftil}{\widetilde{\mathbf{R}}}
% \newcommand{\Rbfbar}{\overline{\mathbf{R}}}
% \newcommand{\rbfbar}{\overline{\mathbf{r}}}
% \newcommand{\rbftil}{\widetilde{\mathbf{r}}}
% \newcommand{\Xbfbar}{\overline{\mathbf{X}}}
% \newcommand{\Wbfbar}{\overline{\mathbf{W}}}
% \newcommand{\Wbftil}{\widetilde{\mathbf{W}}}
% \newcommand{\wbfbar}{\overline{\mathbf{w}}}
% \newcommand{\wbftil}{\widetilde{\mathbf{w}}}
% \newcommand{\xbfbar}{\overline{\mathbf{x}}}

